Super-approximation, II: the p-adic and bounded power of square-free integers cases

Let $\Omega$ be a finite symmetric subset of GL$_n(\mathbb{Z}[1/q_0])$, and $\Gamma:=\langle \Omega \rangle$. Then the family of Cayley graphs $\{{\rm Cay}(\pi_m(\Gamma),\pi_m(\Omega))\}_m$ is a family of expanders as $m$ ranges over fixed powers of square-free integers and powers of primes that are coprime to $q_0$ if and only if the connected component of the Zariski-closure of $\Gamma$ is perfect. Some of the immediate applications, e.g. orbit equivalence rigidity, {\em largeness} of certain $\ell$-adic Galois representations, are also discussed.

==> SG_FiniteLog.tex <==
\subsection{Finite logarithmic maps.}\label{ss:FiniteLog}
Here we recall the {\em finite logarithmic maps} and their main properties. These maps are the key connection between congruence groups and the Lie algebra. All of these results are well-known for Chevalley groups, but I could not find them in the literature in the generality needed for this work.  Let $\bbg\subseteq (\mathbb{SL}_n)_{\bbq}$ be a connected simply-connected perfect $\bbq$-subgroup (notice that a perfect linear algebraic group is automatically a subset of $\mathbb{SL}_n$) and $\gcal$ be its Zariski-closure in $(\mathcal{SL}_n)_{\bbz_S}$; in particular $\gcal$ is a flat finite-type $\bbz_S$-group scheme. 

Let us recall that $\Lie \gcal$ is a $\bbz_S$-group scheme and for any $\bbz_S$-algebra $R$ we have that 
\be\label{e:ExactLieAlgebra}
1\rightarrow \Lie \gcal(R)\rightarrow \gcal(R[x]/\langle x^2\rangle) \rightarrow \gcal(R)\rightarrow 1
\ee
is a short exact sequence. If $\gcal$ is a {\em smooth} $\bbz_S$-group scheme, then $\Lie \gcal=\underline{\gfr}$, where $\gfr=\Lie \gcal(\bbz_S)$ and $\underline{\gfr}(R):=\gfr \otimes_{\bbz_S} R$ for any $\bbz_S$-algebra $R$. On the other hand, since the generic fiber $\bbg$ of $\gcal$ is smooth, there is a finite set of primes $S'\supseteq S$ such that $\gcal\times_{\Spec \bbz_S}\Spec \bbz_{S'}$ is a smooth $\bbz_{S'}$-group scheme, and in particular $\Lie \gcal\times _{\Spec \bbz_S}\Spec \bbz_{S'}=\underline{\gfr}\times_{\Spec \bbz_S}\Spec \bbz_{S'}$.  

To be more precise, suppose $f_1,\ldots,f_s\in \bbz_S[X_{11},\ldots,X_{nn}]$ is a set of defining relations of $\gcal$, i.e. as a $\bbz_S$-scheme $\gcal=\Spec(\bbz_S[X_{11},\ldots,X_{nn}]/\langle f_1,\ldots,f_s\rangle)$. Then as a $\bbz_S$-scheme 
\be\label{e:LieAlgebra}
\Lie \gcal=\Spec(\bbz_S[X_{11},\ldots,X_{nn}]/\langle (df_1)_I,\ldots,(df_s)_I\rangle),
\ee
 where $(df_k)_I(Y_{ij}):=\sum_{ij}(\partial f_k/\partial X_{ij})(I) Y_{ij}$. Looking at the Taylor expansion of $f_i$ we see that for a $\bbz_S$-algebra $R$ and $Y\in {\rm M}_n(R)$ we have $(df_i)_I(Y)=0$ if $f_i(I+tY)=0$ and $t^2=0$ in $R$. Therefore, for $q_1|q_2|q_1^2$, we get the following maps
\[
\wt{\lin{q_1}{q_2}}:\pi_{q_2}(\ker \pi_{q_1})\rightarrow \Lie \gcal(\bbz_S/q_3\bbz_S), \h\h \wt{\lin{q_1}{q_2}}(\pi_{q_2}(g)):=\pi_{q_3}((g-1)/q_1),
\]
where $q_3=q_2/q_1$ and $\pi_q:\gcal(\bbz_S)\rightarrow \gcal(\bbz_S/q\bbz_S)$. Notice that $\Lie \gcal(\bbz_S/q_3\bbz_S)$ is NOT isomorphic to $\gfr/q_3 \gfr$ in general, but this is the case when $q_3$ does not have small prime factors (as it is pointed out above). In fact, by (\ref{e:LieAlgebra}), $\Lie \gcal(R)=\{Y\in {\rm M}_n(R)|\h F(Y)=0\}$ where, $F:\bbz_S^{n^2}\rightarrow \bbz_S^s,\h F(Y)=((df_1)_I(Y),\ldots,(df_s)_I(Y))$. So there is an integer $q_0$ (depending on $f_i$) such that, for any $q\in \bbz_S$, $\Lie\gcal(\bbz_S/q\bbz_S)$ can be naturally mapped onto $\gfr/q^-\gfr$, where $q^-:=q/\gcd(q,q_0)$. Hence for $q_1|q_2|q_1^2$ we get the {\em finite logarithmic maps}: 
\be\label{e:FiniteLogMap}
\lin{q_1}{q_1q_3^-}:\pi_{q_1q_3^-}(\ker \pi_{q_1})\rightarrow \gfr/q_3^-\gfr, \h\h \linValue{q_1}{q_1q_3^-}{g}:=\pi_{q_3^-}(x), 
\ee
where $x\in \gfr\subseteq \mathfrak{sl}_n(\bbz_S)$ and $\pi_{q_3^-}(x)=\pi_{q_3^-}((g-1)/q_1)$. Let $\Gamma$ be a finitely generated subgroup of $\gcal(\bbz_S)$ which is Zariski-dense in $\bbg$. We can and will consider the restriction of the finite logarithmic maps to $\Gamma$. In the next lemma, we summarize the important properties of $\lin{q_1}{q_2}$.


\begin{lem}\label{l:PropertiesOfLinearizationMap}
Let $\Gamma$ and $\gcal$ be as above. Assume $q_1|q_2|q_1^2$, $q_1'|q_2'|q_1'^2$ and $q_1|q_1'$, and let $q=\gcd(q_2q_1',q_1q_2')$. Suppose either $q_3:=q_2/q_1$ and $q_3':=q_2'/q_1'$ have large prime factors (depending on $\Gamma$), or $q_i$ are powers of a single prime $p$ and $\log_p q_1^2/q_2,\log_p q_1'^2/q_2'\gg_{\Gamma} 1$. Then
\begin{enumerate}
	\item $\lin{q_1}{q_2}:\pi_{q_2}(\ker \pi_{q_1})\rightarrow \gfr/q_3\gfr$ is a well-defined, injective additive homomorphism. 
	\item\label{i:Equi} $\lin{q_1}{q_2}$ is $\Gamma$-equivariant, i.e. for any  $\gamma\in \Gamma)$ and $g\in \ker \pi_{q_1}$, there is $x\in \gfr$ such that $\pi_{q_1q_1^-}(g)=\pi_{q_1q_1^-}(1+q_1x)$ and 
\[	
\linValue{q_1}{q_2}{\gamma^{-1} g\gamma}=\pi_{q_3}(\Ad(\gamma)(x)).
\] 
 \item If $g\in \ker \pi_{q_1}$ and $g'\in \ker \pi_{q_1'}$, then $(g,g'):=g^{-1}g'^{-1}gg'\in \ker \pi_{q_1q_1'}$. And 
 \[
 \linValue{q_1q_1'}{q}{(g,g')}=\pi_{q/(q_1q_1')}([\linValue{q_1}{q_2}{g}, \linValue{q_1'}{q_2'}{g'}]),
 \]
 where $[x_1,x_2]:=x_1x_2-x_2x_1$.
 \item In the case when $q_i$ are powers of a prime $p$, if $\log_p q_1\gg_{\Gamma} 1$, then $\lin{q_1}{q_2}$ is an additive group isomorphism; in fact by part (\ref{i:Equi}) it is a $\Gamma$-module isomorphism.
\end{enumerate}
\end{lem}
\begin{proof}
We have already discussed why $\lin{q_1}{q_2}$ is well-defined. And from the definition of $\lin{q_1}{q_2}$ it is an embedding. Now the rest of the claims except the last one can be proved by straightforward computations. 

By strong approximation~\cite{Nor}, $\Gamma$ is dense in an open subgroup of $\gcal(\bbz_p)$. Let 
\[
G(p^m):=\{g\in \gcal(\bbz_p)|\h\pi_{p^m}(g)=1\}.
\]
 Then the exponential map $\exp: p^k\gfr(\bbz_p)\rightarrow G(p^k)$ and the logarithmic map $\log:G(p^k)\rightarrow p^k\gfr(\bbz_p)$ are well-defined analytic functions and inverse of each other for $k\gg 1$; in particular $\|\exp(x)-I\|_p=\|x\|_p$ and $\|\log g\|_p=\|g-I\|_p$. Therefore for any $x\in \gfr(\bbz_p)$ and large enough $k$ (depending on $\Gamma$) we have that $\pi_{p^{2k}}(\exp(p^k x))\in \pi_{p^{2k}}(\Gamma)$. And so $\pi_{p^{2k}}(I+p^kx)\in \pi_{p^{2k}}(\Gamma)$, which implies that $\lin{q_1}{q_2}$ is onto if $\log_p q_1\gg_{\Gamma}1$.  


%Let's see the details of the argument for the third property. Let $x,x'\in \gfr$ such that $g=1+q_1 x \pmod{q_2}$ and $g'=1+q_1' x'\pmod{q_2'}$. We have to show that $(g,g')=1+q_1q_1'[x,x'] \pmod{q}$.
%First notice that $q_1'^3$ is divisible by $q)$. Hence 
%\be\label{e:Inverse1} 
%g'^{-1}=1-q_1'x'+q_1'^2x'^2 \pmod{q}.
%\ee
%We also notice that, since $q$ divides $q_1^2q_1'$ and $q_1'q_2'$, we have
%\be\label{e:Inverse2}
%q_1'g^{-1}=q_1'(1-q_1x)\pmod{q}\h\h\h\text{and}\h\h\h q_1'g'=q_1'(1+q_1'x')\pmod{q}.
%\ee
%Hence we have that 
%\begin{align*}\label{e:Commutator}
%(g,g')&=g^{-1}(1-q_1'x'+q_1'^2x'^2)gg'\pmod{q}\\
%&=(1-q_1'g^{-1}x'g+q_1'^2g^{-1}x_1'^2g)g'\pmod{q}\\
%&=(1-q_1'(1-q_1x)x'(1+q_1x)+q_1'^2(1-q_1x)x'^2(1+q_1x))g'\pmod{q}\\
%&=(1-q_1'x'+q_1q_1'[x,x']+q_1'^2 x'^2)g' \pmod{q}\\
%&=(1-q_1'x')g'+q_1q_1'[x,x'](1+q_1'x')+q_1'^2x'^2(1+q_1'x') \pmod{q}\\
%&=1-q_1'^2x'^2g'+q_1q_1'[x,x']+q_1'^2x'^2 \pmod{q}\\
%&=1-q_1'^2x'^2(1+q_1'x')+q_1q_1'[x,x']+q_1'^2x'^2 \pmod{q}\\
%&=1+q_1q_1'[x,x']  \pmod{q}.
%\end{align*}
\end{proof}

==> SG_TaoBalogSzemerediGowers.tex <==
\section{Prelimanry results}
%%%%%%%%%%%%%%%%%% Bourgain Gamburd Remark %%%%%%%%%%%%%%%%%%%%%%%%
\subsection{}\label{ss:RemarkRandomWalk}
The following is a useful lemma (see~\cite[Remark, page 1060]{BG3}).
\begin{lem}\label{l:BGRemark}
Let $H$ be a group, $\mu$ be a symmetric probability measure on $H$, and $A$ be a symmetric subset of $H$. If $l>l_0$ are two positive integers, then $\mu^{(2l_0)}(A\cdot A)\ge \mu^{(l)}(A)^2$. 
\end{lem}
\begin{proof}
First we notice that, since $\mu^{(l)}(A)=\sum_{h\in H}\mu^{(l-l_0)}(h)\mu^{(l_0)}(h^{-1}A)$, $\mu^{(l)}(A)\le \max_{h\in H}\mu^{(l_0)}(hA)$. Now since $A$ and $\mu$ are symmetric, we also have that $\mu^{(2l_0)}(A\cdot A)\ge \max_{h\in H}\mu^{(l_0)}(hA)^2$. 
\end{proof}

 

%%%%%%%%%%%%%%%%%% Balog Szemeredi Gowers %%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{}\label{ss:BalogSzemerediGowers}
The following is an important lemma~\cite[Lemma 15]{Var} (also see \cite{BG1}) which is based on the non-commutative version of Balog-Szemer\'{e}di-Gowers Theorem~\cite{Tao}. 
\begin{lem}\label{l:BSG}
Let $H$ be a finite group and $\mu$ be a probability measure on $H$. Let $K$ be a positive number. 
If $\|\mu *\mu\|_2\ge \frac{1}{K}\|\mu\|_2$, then there is a subset $A$ of $H$ with the following properties:
\begin{enumerate}
\item $\frac{1}{K^R\|\mu\|_2^2}\le |A|\le \frac{K^R}{\|\mu\|_2^2}$,
\item $|A\cdot A\cdot A|\le K^R |A|$,
\item $\min_{h\in A} (\widetilde{\mu}*\mu)(h)\ge \frac{1}{K^R|A|}$, where $\widetilde{\mu}(h)=\mu(h^{-1})$ for any $h\in H$.
\end{enumerate}
\end{lem}


